Multiplicity Problems on Algebraic Series and Context-Free Grammars

In this paper we obtain complexity bounds for computational problems on algebraic power series over several commuting variables. The power series are specified by systems of polynomial equations: a formalism closely related to weighted context-free grammars. We focus on three problems -- decide whether a given algebraic series is identically zero, determine whether all but finitely many coefficients are zero, and compute the coefficient of a specific monomial. We relate these questions to well-known computational problems on arithmetic circuits and thereby show that all three problems lie in the counting hierarchy. Our main result improves the best known complexity bound on deciding zeroness of an algebraic series. This problem is known to lie in PSPACE by reduction to the decision problem for the existential fragment of the theory of real closed fields. Here we show that the problem lies in the counting hierarchy by reduction to the problem of computing the degree of a polynomial given by an arithmetic circuit. As a corollary we obtain new complexity bounds on multiplicity equivalence of context-free grammars restricted to a bounded language, language inclusion of a nondeterministic finite automaton in an unambiguous context-free grammar, and language inclusion of a non-deterministic context-free grammar in an unambiguous finite automaton.

==> invhom.tex <==

\paragraph{Grammars restricted to a regular letter-bounded language}

The multiplicity semantics of $X$ \emph{restricted} to a language $L \subseteq \Sigma^*$,
written $\restrict {\sem X} L$,
agrees with $\sem X$ on $L$ and is zero otherwise.
%
% Fix any regular letter-bounded language $R \subseteq \sigma_1^* \cdots \sigma_k^*$
%
The multiplicity equivalence problem \emph{restricted} to a language $L \subseteq \Sigma^*$
asks whether $\restrict {\sem X} L = \restrict {\sem Y} L$.

\begin{lemma}
    \label{lem:regular restriction}
    The multiplicity equivalence problem for grammars
    restricted to a regular language $L \subseteq \Sigma^*$
    reduces in polynomial time to the multiplicity equivalence problem for grammars recognising a subset of $L$.
\end{lemma}

\begin{proof}
    Consider a grammar $G$ and a nondeterministic finite automaton $A$ recognising a language $L(A)$.
    %
    It is well-known that context-free languages are closed w.r.t.~intersection with regular languages.
    %
    The usual construction first converts the grammar $G$ and nonterminal $X$
    to a pushdown automaton $P_X$ recognising the same language as $X$,
    and then builds a product $P_X \times A$ recognising $L(P_X) \cap L(A)$.
    %
    These constructions can be done in polynomials time and even respect multiplicities:
    $\sem X = \sem {P_X}$, where the multiplicity semantics of a pushdown automaton $\sem {P_X}$
    counts the number of accepting runs \cite[Theorem 14.33]{KuichSalomaa}.
    %
    When the regular language is presented by a nondeterministic finite automaton $A$,
    the usual product construction (cf.~\cite[Theorem 7.27]{HopcroftMotwaniUllman:2000})
    produces a pushdown automaton $P_X \times A$ \st
    %
    \begin{align*}
        \sem {P_X \times A}_w = \sem {P_X}_w \cdot \sem A_w,
    \end{align*}
    %
    where $\sem A$ is the multiplicity semantics of $A$ counting the number of accepting runs.
    %
    Therefore $X, Y$ are multiplicity equivalent restricted to $L(A)$
    iff $P_X \times A, P_Y \times A$ are multiplicity equivalent.
    %
    Indeed, for every word $w$ we have two cases to consider:
    %
    \begin{enumerate}
        \item If $w \not \in L(A)$, then all quantities
        $(\restrict {\sem X} {L(A)})_w$,
        $(\restrict {\sem Y} {L(A)})_w$,
        $\sem {P_X \times A}_w$, $\sem {P_Y \times A}_w$
        are zero, and we are done.

        \item If $w \in L(A)$, then
        $(\restrict {\sem X} {L(A)})_w = \sem X_w$ and $(\restrict {\sem Y} {L(A)})_w = \sem Y_w$.
        %
        Moreover, in this case $\sem A_w \neq 0$.
        It follows that 
        $(\restrict {\sem X} {L(A)})_w = (\restrict {\sem Y} {L(A)})_w$ iff
        $\sem X_w = \sem Y_w$ iff
        $\sem X_w \cdot \sem A_w = \sem Y_w \cdot \sem A_w$ iff
        $\sem {P_X \times A}_w = \sem {P_Y \times A}_w$. \qedhere
    \end{enumerate}
    %
    Finally, by \cite[Theorem 14.33]{KuichSalomaa} one can construct in polynomial time
    two new nonterminals $\widetilde X, \widetilde Y$
    with the same multiplicity semantics as $P_X \times A$, resp., $P_Y \times A$.
    %
    All in all, we have reduced in polynomial time
    the multiplicity equivalence of nonterminals $X, Y$ restricted to $L(A)$
    to the multiplicity equivalence problem of nonterminals $\widetilde X, \widetilde Y$.
\end{proof}

If we apply the lemma above
to the case when $L \subseteq \sigma_1^* \cdots \sigma_k^*$ is a letter-bounded regular language,
we obtain a reduction to multiplicity equivalence of grammars recognising a letter-bounded language,
and we can thus apply \cref{cor:multiplicity equivalence - letter bounded}.

\begin{corollary}
    \label{cor:restricted multiplicity equivalence - letter bounded}
    The multiplicity equivalence problem for context-free grammars
    restricted to a letter-bounded regular language
    (presented as a nondeterministic finite automaton)
    is polynomial-time reducible to {\EqAlg}.
\end{corollary}

% Notice that letter-bounded context-free languages are not closed under intersection.
% For instance, $L := \setof {a^m b^m c^n}{m, n \in \N}$ and $M := \setof {a^m b^n c^n}{m, n \in \N}$
% are letter-bounded context-free languages $L, M \subseteq a^*b^*c^*$,
% however $L \cap M = \setof {a^m b^m c^m}{m \in \N}$ is not a context-free language.


\subsection{Bounded context-free languages}

In this section we extend the results of the previous section
from letter bounded languages
to the more general class of bounded languages.
%
A language $L \subseteq \Sigma^*$ is \emph{bounded}
if there exist nonempty words $w_1, \dots, w_k \in \Sigma^+$
\st $L \subseteq w_1^* \cdots w_k^*$.

Checking whether a given grammar recognises a bounded language is decidable \cite[Theorem 5.5.2]{Ginsburg:1966}
(even in polynomial time \cite[Theorem 19]{Gawrychowski:Krieger:Rampersad:Shallit:IJFCS:2010}).
%
We note however that there are grammars recognising a bounded language
where the number of witnessing words $k$ is exponential in the size of the grammar.
%
Many algorithmic problems on context-free languages become either decidable,
or their computational complexity is much lower on bounded context-free languages.

\paragraph{Grammars recognising a bounded language}

We show how to decide multiplicity equivalence of two nonterminals $X, Y$
recognising bounded languages $L(X), L(Y) \subseteq w_1^* \cdots w_m^*$.
%
We stress that nonempty words $w_1, \dots, w_m \in \Sigma^+$
are explicitly given in input to the problem.
%
Consider a fresh alphabet $\Gamma = \set{a_1, \dots, a_m}$
and the homomorphism $h : \Gamma^* \to \Sigma^*$
uniquely defined by setting $h(a_1) = w_1, \dots, h(a_m) = w_m$.
%
We associate to a nonterminal $X$ a fresh nonterminal $\widetilde X$ in polynomial time
(together with suitable rules) in order to satisfy the following claim.

\begin{restatable}{lemma}{lemmainvhomo}
    \label{lem:invhomo}
    For every nonterminal $X$ and word $w \in \Gamma^*$, we have
    \begin{align*}
        \sem {\widetilde X}_w = \sem X_{h(w)}.
    \end{align*}
\end{restatable}

\begin{proof}[Proof]
    This is done in three steps.
    %
    In the first step, we convert in polynomial time the nonterminal $X$
    to a pushdown automaton $A$ with the same multiplicity semantics \cite[Theorem 14.33]{KuichSalomaa}:
    $\sem X = \sem A$.
    %
    In the second step, from $A$ we build a pushdown automaton $B$
    recognising the inverse homomorphic image of the language recognised by $A$:
    $L(B) = h^{-1}(L(A))$.
    %
    This can be achieved by a standard construction on pushdown automata
    \cite[Theorem 7.30]{HopcroftMotwaniUllman:2000},
    which can be performed in polynomial time.
    %
    An inspection of the construction allows us to observe that that multiplicities are preserved:
    For every $w \in \Gamma^*$,
    $\sem A_{h(w)} = \sem B_w$
    (cf.~also \cite[Claim 11]{Raz:DLT:1993}).
    %
    In the third step, we convert back in polynomial time the pushdown automaton $B$
    to a nonterminal $\widetilde X$
    having the same multiplicity semantics \cite[Theorem 14.33]{KuichSalomaa}:
    $\sem B = \sem {\widetilde X}$.
\end{proof}

We have thus efficiently reduced the multiplicity equivalence problem for grammars
to the same problem of their inverse homomorphic images.
%
In particular, since the original nonterminals recognise bounded languages $\subseteq w_1^* \cdots w_m^*$,
their inverse homomorphic images recognise letter-bounded languages $\subseteq a_1^* \cdots a_m^*$.
%
We can thus apply \cref{cor:multiplicity equivalence - letter bounded} and obtain the following corollary.

\begin{corollary}
    \label{cor:multiplicity equivalence - bounded}
    The multiplicity equivalence problem for context-free grammars
    recognising a bounded language subset of $w_1^* \cdots w_m^*$ (for given $w_1, \dots, w_m$)
    is polynomial-time reducible to {\EqAlg}.
\end{corollary}

\paragraph{Grammars restricted to a regular bounded language}

Consider a bounded regular language $L \subseteq w_1^* \cdots w_m^*$
and consider the multiplicity equivalence problem for grammars restricted to $L$.
%
By \cref{lem:regular restriction} we can efficiently reduce this problem
to the multiplicity equivalence problem for grammars recognising (bounded) languages $\subseteq L$,
to which we apply \cref{cor:multiplicity equivalence - bounded}.
%
This immediately yields the following corollary.

\begin{corollary}
    \label{cor:restricted multiplicity equivalence - bounded}
    The multiplicity equivalence problem for context-free grammars
    restricted to a bounded regular language subset of $w_1^* \cdots w_m^*$ (for given $w_1, \dots, w_m$)
    is polynomial-time reducible to {\EqAlg}.
\end{corollary}

\newcommand{\ignore}[1]{}

\ignore{  
\subsection{\protect{Proof of \cref{lem:invhomo}}}

A \emph{pushdown automaton} is a tuple $A = \tuple{\Sigma, \Gamma, P, p_0, Z_0, F, \Delta}$
where $\Sigma$ is the input alphabet,
$\Gamma$ is the stack alphabet,
$P$ is a finite set of control locations,
$p_0 \in P$ is the initial location,
$Z_0 \in \Gamma$ is the bottom of stack marker,
$F \subseteq P$ is the set of final control locations,
and $\Delta$ is a set of transition rules of the form
$pX \goesto a q\gamma$,
meaning that from control location $p$ and top-of-stack symbol $X$ (which is popped off the stack)
the automaton can read input symbol $a \in \Sigma \cup \set \e$ (which could be empty)
and go to control location $q$ and push $\gamma$ on top of the stack.

A configuration is a pair $p\gamma$ where $p \in P$ is a control location
and $\gamma \in \Gamma^*$ is the content of the stack.
%
The notion of run over an input $w \in \Sigma^*$
from a configuration $p\gamma$ to a configuration $q\delta$,
written $p\gamma \goesto w q\delta$,
is defined in the standard way.
The run is accepting if $q \in F$.
%
The multiplicity semantics of a configuration $p\gamma$ over an input $w \in \Sigma^*$,
written $\sem {p\gamma}_w$,
is the number of accepting runs from $p\gamma$ over $w$.

\begin{lemma}
    For any context-free grammar $G$ and nonterminal $X$ thereof
    we can construct in polynomial time a pushdown automaton $A$ with initial state $p_0$ and bottom of stack symbol $Z_0$
    \st $\sem X = \sem{p_0 Z_0}$.
\end{lemma}

\begin{proof}
    The standard construction showing that context-free languages are pushdown-recognisable languages
    has the property that multiplicities are preserved.
    %
    A context-free grammar with initial nonterminal $S$
    is the same as a pushdown automaton with a single control location $P = \set{p_0}$,
    which is moreover initial,
    provided we accept by empty stack.
    Acceptance by control location can be achieved by adding an accepting control location $p_f$
    and a single rule $p_0Z_0 \goesto \e p_f Z_0$.
    We also have an initial transition $p_0Z_0 \goesto \e p_0SZ_0$ loading $S$ onto the stack.
    Derivation trees of the grammar are in bijection with left-most derivations,
    which in turn are in bijection with accepting runs of the pushdown automaton from configuration $p_0Z_0$.
\end{proof}

\begin{lemma}
    For any pushdown automaton $A$ with initial state $p_0$ and bottom of stack symbol $Z_0$
    we can construct in polynomial time a context-free grammar $G$ and nonterminal $X$ thereof
    \st $\sem{p_0 Z_0} = \sem X$.
\end{lemma}

\begin{proof}
    The standard construction converting a pushdown automaton to a grammar recognising the same language
    has the property that it preserves multiplicities.
    %
    One considers a nonterminal $\triple p X q$ for every stack symbol $X \in \Gamma$ and control locations $p, q \in P$.
    %
    We can assume that the pushdown automaton either does not push anything on the stack or that it pushes exactly two symbols.
    %
    If the pushdown automaton has a transition rule $pX \goesto a q\e$,
    then the grammar has a rule
    \begin{align*}
        \triple p X q \rightarrow a
    \end{align*}
    If the pushdown automaton has a transition rule $pX \goesto a qYZ$,
    then the grammar has a rule
    %
    \begin{align*}
        \triple p X s \rightarrow a \cdot \triple q Y r \cdot \triple r Z s, \text{for every } r, s \in P.
    \end{align*}
    %
    The nonterminal $\triple p X q$
    recognises the set of all words which are accepted by the pushdown automaton
    when going from control location $p$ and $X$ on top of the stack and ending in control location $q$ and empty stack.
    %
    Moreover, there is a bijection between left-most derivations of words from $\triple p X q$
    and runs from $pX$ to $q\e$.
\end{proof}

\begin{lemma}
    Let $h : \Sigma^* \to \Sigma_1^*$ be a homomorphism.
    For any pushdown automaton $A$ over input alphabet $\Sigma_1$
    we can construct in polynomial time a pushdown automaton $B$ over input alphabet $\Sigma$
    \st for every word $w \in \Sigma^*$,
    $\sem B_w = \sem A_{h(w)}$.
\end{lemma}

\begin{proof}
    The standard construction showing that pushdown-recognisable languages are closed under inverse homomorphic images
    preserves multiplicities.
    %
    Let $\Sigma = \set{\sigma_1, \dots, \sigma_k}$
    and consider a pushdown automaton $A$ with control locations $P$ over input alphabet $\Sigma_1$.
    %
    Consider a homomorphism $h$
    uniquely determined by $h(\sigma_1) = w_1$, \dots, $h(\sigma_k) = w_k$.
    %
    We build a new pushdown automaton $B$ with control locations $Q$
    of the form $\tuple {p, w}$
    where $w$ is a suffix of one of $w_1$, \dots, $w_k$, which we call buffer.
    %
    The automaton $B$ can always replenish an empty buffer, without modifying the stack:
    For every input symbol $\sigma_i \in \Sigma$
    %
    \begin{align*}
        \tuple{p, \e} X \goesto {\sigma_i} \tuple{p, w_i} X.
    \end{align*}
    %
    The automaton simulates a transition $p X \goesto a q \gamma$ of $A$,
    with $a \in \Sigma_1 \cup \set \e$,
    by using the buffer:
    \begin{align*}
        \tuple {p, a w} X \goesto \e \tuple{q, w} \gamma.
    \end{align*}
    %
    If $p_0$ is the start state of $A$,
    then $\tuple {p_0, \e}$ is the start state of $B$.
    If $p$ is a final state of $A$,
    then $\tuple{p, \e}$ is a final state of $B$.
    %
    Let $\sem{pX, q}_u$ be the number of all runs over $u$ starting at $pX$ and ending in $q\e$.
    We then have $\sem A = \sum_{q \in F} \sem{p_0Z_0,q}$.
    \begin{claim}
        For every control locations $p, q$ of $A$, stack symbol $X$,
        and input word $w \in \Sigma^*$, we have
        %
        \begin{align}
            \sem {pX, q}_{h(w)} = \sem {\tuple{p, \e} X, \tuple{q, \e}}_w
        \end{align}
    \end{claim}
    %
    \begin{proof}[Proof of the claim]
        We claim can be proved by induction on the number of steps of the pushdown automata.
    \end{proof}
    %
    The claim implies, as required,
    \begin{align}
        \sem A_{h(w)} = \sem B_w.
    \end{align}

\end{proof}

\lemmainvhomo*

\begin{proof}
    TODO.
\end{proof}

}



==> upperbound.tex <==
An instance  of the evaluation problem comprises a weighted context-free grammar over the unary alphabet~$\{a\}$, a
 positive integer $N$, and a prime number $p$.  
The problem asks to compute the residue modulo $p$ of the weight of the word $a^N$.  In analysing the complexity of the problem we assume that all integers are represented in binary.
In this section we prove the following theorem:
\begin{theorem}\label{thm:coeffslp}
The evaluation problem is in ${\bf \# P}$.
\end{theorem}
The proof is spread across several subsections.
Throughout we work with a  weighted context-free grammar $G=(V, R, S)$ over a unary alphabet~$\{a\}$---forming part of the input to the evaluation problem.
We let $s$ denote the length of the description of the grammar and $d$ the number of nonterminals. 



Associated with the grammar $G$  we have a vector of formal power series 
${\bf A}=(A_1,\ldots,A_d) \in \Q[\![x]\!]^d$ defined by writing
$A_i(x) := \sum_{j = 0}^\infty w_{i,j}x^{j}$, where $w_{i,j}$ is the weight of the word $a^j$ produced starting from the $i$-th non-terminal.  In other words, the sequence $A_i$ is the generating function of $i$-th nonterminal  of $G$.
The evaluation problem asks to compute the 
residue modulo $p$ of the $N$-coefficient 
of the power series  associated to the starting nonterminal of $G$, say $A_1$. This power series will play a central role in the proof of Theorem~\ref{thm:coeffslp}.  Roughly speaking, our strategy is to seek a sufficiently close polynomial approximation of $A_1$ that admits an efficiently computable representation as a circuit.  For this we will exploit a multivariate version of Hensel's Lemma together with a known fixed-point characterisation of ${\bf A}$.


\subsection{Algebraic  Characterisation}
Let~$\{X_1,\cdots, X_d\}$ be an enumeration of the set~$V$ of nonterminals (variables) in $G$, where $X_1$
is the starting nonterminal.
The vector of formal power series 
${\bf A}=(A_1,\ldots,A_d) \in \Q[\![x]\!]^d$
associated to~$G$ satisfies a system of polynomial equations with coefficients in $\Q[x]$.
This system of equations has one variable for each nonterminal.  Here it is convenient to actually take 
$\{X_1,\cdots, X_d\}$ as the set of variables, i.e., we identify each variable with the corresponding nonterminal.  The system of polynomial equations is constructed as follows:
\begin{align}
	X_1 =\, &g_1(X_1, \ldots, X_d) \nonumber
	\\ 
	X_2 =\, &g_2(X_1, \ldots, X_d) \nonumber
	\\ 
	&\vdots \nonumber \\
	X_d =\, &g_n(X_1, \ldots, X_d) \label{eq:gioperator}
\end{align}
where  $g_i \in \Q[x][X_1, \ldots, X_d]$.  For each nonterminal $X_i$, we construct the polynomial $g_i$ as a sum of monomials obtained from the production rules  with $X_i$ as left-hand side. That is, for each production rule $X_i \xrightarrow{k}a \beta$, where $\beta\in V^{*}$, we add a monomial~$k x X_1^{e_1}X_2^{e_2}\cdots X_d^{e_d}$ to $g_i$ where the $e_j$ is the number of times $X_j$ appears in~$\beta$.

By construction, the associated vector~$\vec{A}$ of power series to~$G$ is  a solution to the  polynomial system of equation in~\eqref{eq:gioperator}.
%
Furthermore, if $G$ is written in the Greibach normal form, its polynomial system is proper in the sense of~\cite[Theorem~1.1 in Chapter~4]{salomaa1978automata}, and  
$\vec{A}$ is the unique solution of~\eqref{eq:gioperator} in the ring~$\Q[[x]]^d$. We reiterate a proof of this well-known fact in~\Cref{app:unique_fixed_point}, by showing that the polynomial mapping~$\vec{g}$ is a contraction in the metric space~$(\Q[[x]]^d, |.|)$, where $|.|$ is the generalisation of the non-archimedean absolute value from $K$ to $K^d$. 

Below, we write $f_i(X_1,\ldots,X_n) = X_i - g_i(X_1,\ldots,X_n)$. We denote by 
\begin{equation}\label{eq:system_f}
	\mathbf{f} = 
	\begin{bmatrix} f_1 \\ \vdots \\ f_n \end{bmatrix}.
\end{equation}


 
 \subsection{Approximation by Rational Functions}
 \label{sec:rational}
  We apply the multidimensional version of Hensel's Lemma to obtain a sequence~$({\bf a})_n$ 
 that converges to ${\bf A}$ in $\mathbb{Q}(x)^d$.
 The sequence is defined inductively by ${\bf a}_0 = {\bf 0}$ and
 \begin{eqnarray*}
{\bf a}_{n+1} &=& {\bf a}_n + (D{\bf f})({\bf a}_n)^{-1} {\bf f}({\bf a}_n)\\
&=& {\bf a}_n +  \frac{1}{J_{\bf f}({\bf a}_{n})}\left(\mbox{Adj}(D{\bf f}({\bf a}_{n})) {\bf f}({\bf a}_n)\right)
\end{eqnarray*}
where $D{\bf f} = \left(\frac{\partial f_i}{\partial X_j}\right)_{i,j \in [d]}$ is a matrix whose entries are formal polynomials in the ring $\mathbb{Q}(x)[X_1, \dots, X_d]$ and $J_{\bf f}$ is the determinant of $D{\bf f}$. 

\textcolor{red}{Check that the conditions of Hensel's Lemma--all lemmas showing that why it works}

By Theorem \ldots we have 
\begin{gather}
	v(A_i - {\bf a}_{n,i}) \geq 2^n
\label{eq:convergence}
\end{gather}
for all $n \in \mathbb{N}$ and all
$i \in \{1,\ldots,d\}$.

\subsection{Approximation by Polynomials}
\label{sec:polynomial}
Note that each approximant ${\bf a}_n \in \mathbb{Q}(x)^d$
in Section~\ref{sec:rational} is a vector of rational functions.
Let us write ${\bf a}_{n,i}(x) = \frac{g_{n,i}(x)}{h_{n,i}(x)}$ where $g_{n,i}(x)$
and $h_{n,i}(x) \in \mathbb{Q}[x]$. \textcolor{red}{Ambiguous! not unique, fix it.}
We next define a sequence $\widetilde{\bf a}_{n} \in \mathbb{Q}[x]^d$ of vectors of polynomials that satisfies the following convergence bound for all $n$
(cf.~Equation~\ref{eq:convergence}):
\begin{gather}
	v(A_i - \widetilde{\bf a}_{n,i}) \geq 2^n
\label{eq:convergence2}
\end{gather}
The definition of $\widetilde{\bf a}_{n,i}$ 
uses a classical technique of division elimination by Strassen~\cite{..}.  To apply this we will need the 
following claim whose proof can be found in Section $\cdots$.

\begin{claim}
\label{clm:hensel_denominator_const1}
For every $i \in [d]$, and $n \in \mathbb{N}$, $ h_{n,i}(0) = 1$.
\end{claim}

By Claim~\ref{clm:hensel_denominator_const1},
for every $i \in [d]$, and $n \in \mathbb{N}$ there exists a polynomial $f_{n,i}(x) \in \mathbb{Q}[x]$ such that $h_{n,i}(x) = 1-xf_{n,i}(x)$.
We now have
\[ {\bf a}_{n,i}(x) = \frac{g_{n,i}(x)}{1- xf_{n,i}(x)} = 
g_{n,i}(x) \sum_{j=0}^\infty (xf_{n,i}(x))^j \, .\]
The definition of $\widetilde{\bf a}_{n,i}$ is obtained by a suitable truncation of the infinite sum above.  We write
\[ \widetilde{\bf a}_{n,i}(x):= 
g_{n,i}(x) \sum_{j=0}^{2^n-1} (xf_{n,i}(x))^j \, . \]
Then we have 
\begin{align*}
    v\left({\bf a}_{n,i} - \tilde{\bf a}_{n,i} \right)
    & = v\left(g_{n,i} \sum_{j=2^n}^{\infty} (xf_{n,i})^j \right) \\
    & = v\left(g_{n,i} \right) + v\left( \sum_{j=2^n}^{\infty} (xf_{n,i})^j \right)\\
    &\geq  2^n \, ,
\end{align*}
where in the last line we use the fact that
$v(g_{n,i}) \geq 0$ and $v(f_{n,i}) \geq 0$.

The desired bound given by Equation~\eqref{eq:convergence2} now follows from~\eqref{eq:convergence} and the strong triangle equality.

\subsection{Approximation by Circuits}
In this section we show that for $i \in [d]$ each of the polynomial approximants 
$\widetilde{\bf a}_{n,i}$ defined in Section~\ref{sec:polynomial} is represented by a circuit that can be computed in time polynomial in $n$ and the size $s$ of the grammar.
We construct the circuit in two steps.  First 
we show how to construct circuits for polynomials $g_{n,i}(x)$ and $h_{n,i}(x)$ 
such that ${\bf a}_{n,i} = \frac{g_{n,i}(x)}{h_{n,i}(x)}$.

\begin{proposition}
\label{prop:newton_rat_function}
Given $n \in \mathbb{N}$ and $i \in [d]$ one can compute in $\poly(s,n)$ time, division-free circuits $C_{n,i}, D_{n,i}$ of size at most $\poly(s, n)$ that compute 
polynomials $g_{n,i}(x),$ $h_{n,i}(x) \in \mathbb{Q}[x]$ respectively, such that ${\bf a}_{n,i}(x) = \frac{g_{n,i}(x)}{h_{n,i}(x)}$.
\end{proposition}

\begin{proof}
Recall that ${\bf a}_0 = \bf 0$ and that we have the recursive formula 
\begin{eqnarray}
{\bf a}_{n+1} &=& {\bf a}_n +  \frac{1}{J_{\bf f}({\bf a}_{n})}\left(\mbox{Adj}(D{\bf f}({\bf a}_{n})) {\bf f}({\bf a}_n)\right) \, ,
\label{eq:update}
\end{eqnarray}
%
where $D{\bf f} = \left(\frac{\partial f_i}{\partial X_j}\right)_{i,j \in [d]}$ is a matrix whose entries are formal polynomials in the ring $\mathbb{Q}(x)[X_1, \dots, X_d]$ and $J_{\bf f}$ is the determinant of $D{\bf f}$. 

We define the circuits $C_{n,i}$ and $D_{n,i}$ 
by induction on $n$.  For each non-terminal $i \in [d]$ we define 
$C_{0,i}$ to be the constant $0$ and $D_{0,i}$ to be the constant $1$. 
For the inductive step we show how to construct for each $i \in [d]$ 
the circuits $C_{n+1,i}$ and $D_{n+1,i}$ from the collection of circuits 
$\{C_{n,j},D_{n,j} : j \in [d]\}$, in time 
${\bf poly}(s)$.  For this we will use Equation~\eqref{eq:update}.  

It is well-known~\cite{berkowitz, mahajan-vinay} 
that for a $(d \times d)$ matrix whose entries are distinct indeterminates there is an algorithm that runs in $\poly(d)$-time and produces
an algebraic circuit that represents the determinant of the matrix.
 This directly yields $\poly(s)$-size circuits for the Jacobian $J_{\bf f}({\bf a}_{n})$ as well as every entry of adjugate $\mbox{Adj}(D{\bf f}({\bf a}_{n}))$ (whose entries are just cofactors of $D{\bf f}$).
 Composing the circuits so-obtained with the circuits  
 $\{C_{n,j},D_{n,j} : j \in [d]\}$
 that represent the respective numerators and denominators of the entries of ${\bf a}_n$ we obtain the desired circuits $C_{n+1,i}$ and $D_{n+1,i}$.
\end{proof}

 
  
  
  \begin{proposition}
\label{prop:poly_circuit}
Given $n \in \mathbb{N}$ and $i \in [d]$ one can compute in $\poly(s,n)$ time, division-free circuits $E_n$ of size at most $\poly(s, n)$ that compute 
polynomials $\widetilde{\bf a}_{n,1}$.
\end{proposition}
\begin{proof}
By definition we have $\widetilde{\bf a}_{n,1}=g_{n,1} \sum_{j=0}^{2^n-1} (xf_{n,1})^j$.  Note that a naive circuit for the expression on the right-hand side would have size $\poly(s)2^n$. However one can build a circuit of size $\poly(s,n)$ by plugging in $y = xf_{n,1}$, and $\ell = 2^n$ in the circuit from Proposition~\ref{prop:gpcircuit}, which concludes our proof.
 \end{proof}


	





